Disaggregated Database Management Systems

Modern applications demand high performance and cost efficient database management systems (DBMSs). Their workloads may be diverse, ranging from online transaction processing to analytics and decision support. The cloud infrastructure enables disaggregation of monolithic DBMSs into components that facilitate software-hardware co-design. This is realized using pools of hardware resources, i.e., CPUs, GPUs, memory, FPGA, NVM, etc., connected using high-speed networks. This disaggregation trend is being adopted by cloud DBMSs because hardware re-provisioning can be achieved by simply invoking software APIs. Disaggregated DBMSs separate processing from storage, enabling each to scale elastically and independently. They may disaggregate compute usage based on functionality, e.g., compute needed for writes from compute needed for queries and compute needed for compaction. They may also use disaggregated memory, e.g., for intermediate results in a shuffle or for remote caching. The DBMS monitors the characteristics of a workload and dynamically assembles its components that are most efficient and cost effective for the workload. This paper is a summary of a panel session that discussed the capability, challenges, and opportunities of these emerging DBMSs and disaggregated hardware systems.

==> hwIntroOLD.tex <==
Composable disaggregated infrastructure (CDI) software and solutions provides an opportunity to rethink data center architectures to accommodate next-generation applications in artificial intelligence & machine learning (AI+ML), high-performance computing (HPC), edge computing, digital media, and other valuable, rapidly evolving technologies. 

These modern workloads have exposed the Achilles heel of traditional server architectures: the sheet metal that surrounds them. With GPU, storage and/or FPGA resource requirements, success is effectively limited to what can fit in a box. Customers are forced to purchase larger, more expensive servers than needed for new deployments or remove and replace when a server is maxed-out.  

In addition, these systems take weeks to order and deploy. This also interrupts the typical refresh cycle for servers due to the extra cost, and other business outlays such as software licensing for the larger servers as well as power/cooling/space constraints in the data center.

Dynamically configured infrastructure is the clear direction of the market, matching workloads with hardware configurations via software, at bare metal, as required, for cloud-like performance regardless of where physical hardware resides.

CDI extracts value from the datacenter by applying a new architecture to conventional servers and their resources.
With any new technology, there are some new concepts that must be learned, and with CDI it can be broken down into three:
\begin{itemize}
    \item The disaggregation of a datacenter’s constituent infrastructure.
    \item A fabric to connect those disaggregated components.
    \item Software that allows the configuration, deployment and scaling of bare-metal systems. 
\end{itemize}
This section describes approaches by Fungible and Liqid in turn.


